ETCetera: beyond Event-Triggered Control

We present ETCetera, a Python library developed for the analysis and synthesis of the sampling behaviour of event triggered control (ETC) systems. In particular, the tool constructs abstractions of the sampling behaviour of given ETC systems, in the form of timed automata (TA) or finite-state transition systems (FSTSs). When the abstraction is an FSTS, ETCetera provides diverse manipulation tools for analysis of ETC's sampling performance, synthesis of communication traffic schedulers (when networks shared by multiple ETC loops are considered), and optimization of sampling strategies. Additionally, the TA models may be exported to UPPAAL for analysis and synthesis of schedulers. Several examples of the tool's application for analysis and synthesis problems with different types of dynamics and event-triggered implementations are provided.

==> Figures/sched_inputs.tex <==
\begin{tikzpicture}
	\begin{axis}[height=0.2\textheight, width=0.5\textwidth, my axis style, axis x line=bottom, axis y line=left, ylabel= Input, xlabel=Time(s), grid=both]
		\addplot[my linestyle, thick, blue] table[y=u1, x=t, col sep=comma]{Figures/sim.csv};
		\addplot[my linestyle, thick, red] table[y=u2, x=t, col sep=comma]{Figures/sim.csv};
	\end{axis}
\end{tikzpicture}

==> Rebuttal/paper_rebuttal_shorter.tex <==
We would like to express our gratitude for all the reviewers’ valuable comments. Find below some responses:

-Reviewers 1 and 2 ask why there is no comparison with software that provides similar functionalities. The reason is that there is no other tool that does any of the following: a) constructs abstractions capturing the sampling behavior of ETC systems, b) analyzes quantitatively ETC’s sampling performance, and c) schedules ETC traffic in shared networks. 

-A discussion on CPU times, computational complexity and scalability is indeed missing. 

Regarding theoretical scalability and complexity: 
1. The size of the state-space partition using either gridding or by IMs+cones scales exponentially with the state-space dimension n. Nonetheless, in the case of linear PETC, the use of isochronous sets removed the dependence on dimensions, and the number of regions r is O(k_{max}^l). 
2. The complexity of IM-approximations mainly depends on the complexity of the SMT solver dreal, which, if we are correct, is exponential on n for our type of problems. 
3. For linear PETC, the transition relation computation is O(Kr^2)C, where C is polynomial in n when using solver='sdr' (see [13]) and exponential in n when using z3 (see [15]). 
4. Generating timing intervals and transitions (in the case of general nonlinear systems) is O(r)C and O(r^2)C respectively, where r is the number of regions and C is the complexity of the reachability analysis tools that are used. 
5. The resulting system \hat{S} for linear PETC has O(k_{max}^{l+1}) states (which is rk_{max}) and O(K^{2l+2}) transitions (which is rk_{max}^2). In practice, the number of regions often grows much slower than exponentially with l, a phenomenon we are currently investigating. 
6. When it comes to scheduling, using UPPAAL the size of the problem scales exponentially with the number of systems in the network (TA safety games are exponential on the number of clocks). The scheduling technique described in section 3.3 is more efficient than that, as it exploits the fact that PETC models are already FSTSs. 

Additionally, partitioning can reduce the number of states to O(k_{max}) (and the transitions accordingly to O(k_{max}^2). However, if the safety game fails, refinement has to be performed, increasing the number of states, and subsequently increasing the cost of the safety game. Introducing BDDs complicates this analysis, see [40] for more details. 

Overall, there is exponential dependence on the number of systems, when it comes to scheduling, and on the system-dimensions (except for linear PETC), when it comes to abstracting, as in most abstraction-based approaches. One way to address the exponential dependence on dimensions is extending the traffic models of linear PETC to general nonlinear systems, which is listed in our future work. 

We need to emphasize that the tool is amenable to severe parallelization (currently work in progress) and the tool is conceived for offline use, with the eventually synthesized scheduler’s online implementation being simply a set of if-then-else rules. 

Regarding real CPU times, we included those in the REP for each example provided. Generating an abstraction for a nonhomogeneous system (IM-based partitioning) takes <1 hour; for a perturbed system with grid partitioning <1 hour; for a 4-dimensional linear system using solver='sdr' 10-20 mins; generating a scheduler via a safety game 10-20 mins; and quantitative analysis on a linear PETC system <5mins. These will be reported the final version.

-Regarding Figure 6: 
Figure 6a shows the lower and upper bounds on inter-event times for each region R_{i,j}, and Figure 6b depicts transitions between regions (a cross at (x,y) indicates a transition from region x to region y). Blue crosses on 6b have been obtained as described in Section 3.1. The indices of regions are of the form (i,j) indicating that the region is confined between the i-th and (i+1)-th IMs (innermost regions are confined only by the i-th manifold) and lies inside the j-th cone.

Reviewer 1:

-Concerns about third-party tools: 
the most important third-party tools that have to be installed by the user (because they are not in Python) are dReal, dReach and Flow*. These are open-source tools and their installation is easy. UPPAAL can also be installed by the user and it is free for academic purposes. We have provided pointers on how to install them on the Gitlab page of ETCetera, and are working on automating their installation.

Reviewer 2:

-On the ball-segment approximations: 
Approximating IMs by ball-segments is easy due to the particular set representation of IMs, see [19]. Nonetheless, (polynomial) zonotopic approximations would definitely be less conservative and are part of current investigations.

-On the disturbance d: 
d is of arbitrary dimensions and has to belong to a hyper-rectangle D.

-“In page 5, it is not clear why (9) is substituted by R_i\rightarrow i R_j for verification.":
We should have stated explicitly "for quantitative verification": when computing the performance of PETC (§3.4), we consider the nominal PETC without early-triggers. Thus, a state in region i always triggers at time h*i. 

-'Also, in page 5, “Note that using relaxations for an existence problem such as the one above” might be nice to explicitly state which it is': 
agreed, it is (9).

Reviewer 4:

-“In section 4.5, in the first lines of the section, the equation used for the state prediction after h times is not consistent with eq. (7).“ 

They are slightly different but they are consistent. The prediction in (7) is sample-by-sample; we are only interested in knowing the sample \hat\xi(t_{i+1}) given the current sample \hat\xi(t_i). In contrast, the prediction in §4.5 is one-step-ahead and based on the current measurement \xi(t) and \hat\xi(t). If you apply the latter recursively from a sampling time, i.e. when \xi(t) = \hat\xi(t), you arrive at (7). 

